Causally Perturbed Fairness Testing

To mitigate unfair and unethical discrimination over sensitive features (e.g., gender, age, or race), fairness testing plays an integral role in engineering systems that leverage AI models to handle tabular data. A key challenge therein is how to effectively reveal fairness bugs under an intractable sample size using perturbation. Much current work has been focusing on designing the test sample generators, ignoring the valuable knowledge about data characteristics that can help guide the perturbation and hence limiting their full potential. In this paper, we seek to bridge such a gap by proposing a generic framework of causally perturbed fairness testing, dubbed CausalFT. Through causal inference, the key idea of CausalFT is to extract the most directly and causally relevant non-sensitive feature to its sensitive counterpart, which can jointly influence the prediction of the label. Such a causal relationship is then seamlessly injected into the perturbation to guide a test sample generator. Unlike existing generator-level work, CausalFT serves as a higher-level framework that can be paired with diverse base generators. Extensive experiments on 1296 cases confirm that CausalFT can considerably improve arbitrary base generators in revealing fairness bugs over 93% of the cases with acceptable extra runtime overhead. Compared with a state-of-the-art approach that ranks the non-sensitive features solely based on correlation, CausalFT performs significantly better on 64% cases while being much more efficient. Further, CausalFT can better improve bias resilience in nearly all cases.

==> Figure/global.tex <==
% \usepackage{CJK}
% \usepackage[top=2cm, bottom=2cm, left=2cm, right=2cm]{geometry}
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}
% \usepackage{amsmath}
% \usepackage[margin=4cm]{geometry}
% \usepackage{algpseudocode}
% \usepackage{algorithm}
% \floatname{algorithm}{Algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{input:}}
% \renewcommand{\algorithmicensure}{\textbf{output:}}

\begin{algorithm}[hbt!]
\caption{Global Generation}
\label{alg:global}
\begin{algorithmic}
\Require Training set $X$, model under test $\mathcal{N}$, protected attributes set $P$, input domain $\mathcal{I}$, $c_{num}$, $g_{num}$, $\eta$, $max_{iter}$, $s_g$

\Ensure Diverse seeds $g_{id}$ violating individual fairness.

\State $g_{id} = \emptyset$

\State $clusters = Clustering(X, c_{num})$

\For{$i$ from $0$ to $g_{num}$}

    \State Sample a seed $x$ from clusters in a round-robin fashion
    
    \State $m = m' = ZerosLike(x)$
    
    \For{$iter$ from $0$ to $max_{iter}$}
    
        \State $similar\_x = \{ x' \in \mathcal{I} | \exists s,r \in P, x'_s \neq x_s ,x'_r \neq x_r; \forall a,r \in A \setminus P, x'_a = x_a \}$
        
        \If{$x$ violates individual fairness}
            \State $g_{id} = g_{id} \cup x$
            
            \State \textbf{Break}
            
        \EndIf
        
        \State $x' = \arg\max_{x' \in similar\_x} \| \mathcal{F}(x) - \mathcal{F}(x') \|_2$
        
        \State $m = \eta \cdot m + \frac{\partial \mathcal{F}(x)}{\partial x}$
        
        \State $m' = \eta \cdot m' + \mathcal{F}(x')_{pred} \cdot \frac{\partial \mathcal{F}(x')_{pred}}{\partial x'}$
        
        \State $dir = ZerosLike(x)$
        
        \For{$a \in A \setminus P$}
        
            \If{$sign(m_a) = sign(m'_a)$ }
                
                \State $dir_a = (-1) \cdot sign(m_a)$
            \EndIf
        \EndFor
        
        \State $x = x + s_g \cdot dir$
        
        \State $x = Clip(x, \mathcal{I})$
    \EndFor
\EndFor

\State \Return $g_{id}$
\end{algorithmic}
\end{algorithm}

==> Figure/local.tex <==
% \usepackage{amsmath}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{amsfonts}

% \begin{document}

\begin{algorithm}
\caption{Local Generation}
\label{alg:local}
\begin{algorithmic}
\Require Model under test $\mathcal{N}$, protected attributes set $P$, input domain $\mathcal{I}$, $g_{id}$, $l_{num}$, $s_l$, $update\_interval$

\Ensure Individual discriminatory instances $l_{id}$.

\State $l_{id} = \emptyset$

\For{$x \in g_{id}$}

    \State $counts = update\_interval$
    
    \For{$i$ from $0$ to $l_{num}$}
    
        \If{$counts = update\_interval$}
        
            \State $similar\_x = \{ x' \in \mathcal{I} | \exists s,r \in P, x'_s \neq x_s ,x'_r \neq x_r; \forall a,r \in A \setminus P, x'_a = x_a ,x'_r = x_r\}$
            
            \State Select $x' \in \{x' \in similar\_x | \mathcal{N}(x) \neq \mathcal{N}(x') \}$
            
            \State $grad = \frac{\partial \mathcal{F}(x)_{pred}}{\partial x}$
            
            \State $grad' = \frac{\partial \mathcal{F}(x')_{pred}}{\partial x'}$
            
            \State $prob = Normalization(grad, grad', P)$
            
            \State $counts = 0$
            
        \EndIf
        
        \State $counts = counts + 1$
        
        \State Select $a \in A \setminus P$ with probability $prob_a$
        
        \State Select $dir \in \{-1, 1\}$ with uniform probability
        
        \State $x_a = x_a + s_l \cdot dir$
        
        \State $x = Clip(x, \mathcal{I})$
        
        \If{$x$ violates individual fairness}
            \State $l_{id} = l_{id} \cup x$
        \Else
            \State Reset($x$); Reset($prob$)
            
            \State $counts = 0$
        \EndIf
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}

% \end{document}

==> Figure/rq3.tex <==

\begin{figure}[t!]
\centering


     \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/adult_sex.pdf}

     \end{subfigure}
~
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/adult_sex.pdf}

        
     \end{subfigure}
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/adult_race.pdf}

     \end{subfigure}
~    
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/compas_sex.pdf}
 
     \end{subfigure}
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/compas_race.pdf}

          
     \end{subfigure}
     ~
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/Lawschool_race.pdf}
          \vspace{-0.6cm}

    \end{subfigure}
 
    \begin{subfigure}[t!]{0.45\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figure/rq3/Lawschool_sex.pdf}
          \vspace{-0.6cm}
          
     \end{subfigure}
 
%     \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/KDD_race.pdf}
%           \vspace{-0.6cm}
         
%      \end{subfigure}
%      ~
%         \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/KDD_sex.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
% ~
%          \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/Dutch_age.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
%        \vspace{-0.2cm}
% ~
%     \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/Dutch_sex.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
%      ~
%         \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/Credit_sex.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
%      ~
%          \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/Credit_education.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
%        \vspace{-0.2cm}
% ~
%     \begin{subfigure}[t]{0.25\columnwidth}
%           \centering
%           \includegraphics[width=\columnwidth]{Figure/rq3/Credit_marriage.pdf}
%           \vspace{-0.6cm}
%      \end{subfigure}
    

      \vspace{-0.3cm}
    \caption{Effect of Dataset Size on IDI in Six generator.}
    \label{fig:size}
\end{figure}


==> Table/rq1-new1.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\caption{Comparing different generators with and without \approach~over all cases using the mean (standard deviation) of individual/group fairness metrics under 10 runs. $f_s$ denotes the concerned sensitive feature. \setlength{\fboxsep}{1.5pt}\colorbox{teal!40}{green cells} mean a generator with \approach~leads to higher IDI ratio/EOD/SPD (hence better at finding fairness bugs) with $p<0.05$ and non-trivial $\mathbf{\hat{A}_{12}}$; \setlength{\fboxsep}{1.5pt}\colorbox{red!20}{red cells} denote a generator without \approach~can better reveal fairness bugs with $p<0.05$ and non-trivial $\mathbf{\hat{A}_{12}}$. Statistically insignificant comparisons (i.e., $p \geq 0.05$ or trivial $\mathbf{\hat{A}_{12}}$) have no rendered color regardless of the results.}

\label{tb:rq1}
\setlength{\tabcolsep}{.7mm}
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{lll|rrr|rrr|rrr|rrr|rrr|rrr} 
\toprule
\multirow{2}{*}{\textbf{Dataset}}   & \multirow{2}{*}{\textbf{$f_s$}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Approach}}} & \multicolumn{3}{c|}{\texttt{ADF}}                                                       & \multicolumn{3}{c|}{\texttt{EIDIG}}                                                     & \multicolumn{3}{c|}{\texttt{NeuronFair}}                                                & \multicolumn{3}{c|}{\texttt{SG}}                                                        & \multicolumn{3}{c|}{\texttt{ExpGA}}                                                     & \multicolumn{3}{c}{\texttt{BREAM}}                                                      \\ 
\cline{4-21}
                           &                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l}{SPD}                                            \\ 
\midrule
\multirow{6}{*}{\textsc{Adult}}     & \multirow{2}{*}{\textit{Gender}}            & w/o \approach
&.291(.003)&\cellcolor{teal!40}{.124(.003)}&\cellcolor{teal!40}{.086(.003)}
&.333(.004)&.114(.004)&\cellcolor{teal!40}{.097(.003)}
&\cellcolor{teal!40}{.351(.004)}&\cellcolor{teal!40}{.138(.003)}&.115(.003)
&\cellcolor{teal!40}{.241(.003)}&\cellcolor{teal!40}{.064(.002)}&.082(.010)
&\cellcolor{teal!40}{.266(.003)}&\cellcolor{teal!40}{.068(.004)}&\cellcolor{teal!40}{.064(.003)}
&.270(.003)&.077(.003)&.076(.003)\\ 

                           &                                 & w/ \approach                     
                           &.301(.003)                   &\cellcolor{teal!40}{.142(.003)}                   &\cellcolor{teal!40}{.103(.003)}       
                           &.316(.003)                   &.169(.003)                   &\cellcolor{teal!40}{.120(.003)}                   
                           &\cellcolor{teal!40}{.365(.004)}                   &\cellcolor{teal!40}{.154(.002)}                   &.137(.003)                   
                           &\cellcolor{teal!40}{.262(.003)}                   &\cellcolor{teal!40}{.127(.003)}                   &.116(.003)                   
                           &\cellcolor{teal!40}{.274(.003)}                   &\cellcolor{teal!40}{.092(.003)}                   &\cellcolor{teal!40}{.104(.002)}                   
                           &.284(.003)                   &.109(.003)                   &.121(.003)   \\        

\cline{3-21}
                           & \multirow{2}{*}{\textit{Race}}           & w/o \approach                          &\cellcolor{teal!40}{.361(.002)}&\cellcolor{teal!40}{.105(.003)}&\cellcolor{teal!40}{.102(.003)}
                           &.382(.003)&\cellcolor{teal!40}{.110(.002)} &\cellcolor{teal!40}{.110(.003)}
                           &.413(.003)&\cellcolor{teal!40}{.120(.003)}&.124(.003)
                           &.238(.003)&\cellcolor{teal!40}{.064(.003)}&\cellcolor{teal!40}{.071(.003)}
                           &\cellcolor{teal!40}{.240(.002)}&.067(.003)&.061(.002)
                           &\cellcolor{teal!40}{.299(.003)}&\cellcolor{teal!40}{.081(.003)}&\cellcolor{teal!40}{.076(.002)}                                   \\   

                           &                                 & w/ \approach                                      
                           &\cellcolor{teal!40}{.382(.003)}&\cellcolor{teal!40}{.113(.003)}&\cellcolor{teal!40}{.132(.003)}
                           &.396(.003)&\cellcolor{teal!40}{.131(.003)} &\cellcolor{teal!40}{.145(.003)}
                           &.429(.003)&\cellcolor{teal!40}{.154(.002)}&.155(.003)
                           &.249(.003)&\cellcolor{teal!40}{.102(.003)}&\cellcolor{teal!40}{.116(.003)}
                           &\cellcolor{teal!40}{.251(.003)}&.079(.003)&.079(.001)
                           &\cellcolor{teal!40}{.316(.003)}&\cellcolor{teal!40}{.086(.002)}&\cellcolor{teal!40}{.097(.003)}  
                           \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Age}}            & w/o \approach  
                           &\cellcolor{teal!40}{.327(.002)}&\cellcolor{teal!40}{.103(.002)}&\cellcolor{teal!40}{.098(.003)}
                           &.343(.003)&.119(.002)&.106(.003)
                           &\cellcolor{teal!40}{.365(.003)}&.139(.002)&.116(.002)
                           &\cellcolor{teal!40}{.250(.003)}&\cellcolor{teal!40}{.061(.002)}&\cellcolor{teal!40}{.071(.003)}
                           &.274(.003)&\cellcolor{teal!40}{.063(.002)}&\cellcolor{teal!40}{.065(.003)}
                           &.296(.003)&.071(.003)&\cellcolor{teal!40}{.071(.003)} 
                                      \\ 

                           &                                 & w/ \approach                                
                           &\cellcolor{teal!40}{.353(.003)}&\cellcolor{teal!40}{.111(.002)}&\cellcolor{teal!40}{.117(.003)}                    
                           &.357(.002)&.113(.004)&.104(.003)                   
                           &\cellcolor{teal!40}{.388(.003)}&.209(.004)&.122(.003)                          
                           &\cellcolor{teal!40}{.251(.003)}&\cellcolor{teal!40}{.122(.003)}&\cellcolor{teal!40}{.098(.003)}                   
                           &.274(.003)&\cellcolor{teal!40}{.056(.003)}&\cellcolor{teal!40}{.069(.003)}                   
                           &.308(.003)&.063(.002)&\cellcolor{teal!40}{.074(.003)}                                   \\ 
                           \hline
                           
\multirow{4}{*}{\textsc{Compas}}    & \multirow{2}{*}{\textit{Gender}}            & w/o \approach 
&\cellcolor{teal!40}{.364(.003)}&\cellcolor{teal!40}{.102(.002)}&\cellcolor{teal!40}{.085(.002)}
&.381(.002)&\cellcolor{teal!40}{.122(.002)}&.092(.002)
&.425(.003)&\cellcolor{teal!40}{.136(.003)}&\cellcolor{teal!40}{.098(.003)}
&\cellcolor{teal!40}{.210(.003)}&.061(.002)&\cellcolor{teal!40}{.054(.003)}
&\cellcolor{teal!40}{.269(.002)}&.067(.003)&\cellcolor{teal!40}{.068(.002)}
&.335(.003)&.056(.003)&\cellcolor{teal!40}{.064(.003)} 
\\ 

                           &                                 & w/ \approach                                    
&\cellcolor{teal!40}{.386(.003)}                   &\cellcolor{teal!40}{.144(.003)}                   &\cellcolor{teal!40}{.130(.002)}                   
&.394(.003)                   &\cellcolor{teal!40}{.157(.003)}                   &.124(.003)                   
&.419(.003)                   &\cellcolor{teal!40}{.163(.003)}                   &\cellcolor{teal!40}{.153(.003)}                   
&\cellcolor{teal!40}{.247(.003)}                   &.103(.002)                   &\cellcolor{teal!40}{.094(.003)}                  
&\cellcolor{teal!40}{.272(.003)}                   &.092(.003)                   &\cellcolor{teal!40}{.105(.003)}                   
&.335(.003)                   &.110(.003)                   &\cellcolor{teal!40}{.126(.003)}                                                           \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Race}}           & w/o \approach                                     
                           &\cellcolor{teal!40}{.418(.002)}&\cellcolor{teal!40}{.104(.003)}&\cellcolor{teal!40}{.084(.002)}
                           &\cellcolor{teal!40}{.426(.003)}&.119(.003)&\cellcolor{teal!40}{.091(.002)}
                           &.472(.003)&\cellcolor{teal!40}{.141(.003)}&\cellcolor{teal!40}{.107(.003)}
                           &.240(.003)&\cellcolor{teal!40}{.050(.003)}&\cellcolor{teal!40}{.066(.003)}
                           &\cellcolor{teal!40}{.286(.003)}&\cellcolor{teal!40}{.056(.002)}&\cellcolor{teal!40}{.083(.003)}
                           &\cellcolor{teal!40}{.343(.004)}&\cellcolor{teal!40}{.068(.003)}&.077(.003)                                     
                           \\ 

                           &                                 & w/ \approach                                      
                           &\cellcolor{teal!40}{.426(.003)}&\cellcolor{teal!40}{.138(.002)}&\cellcolor{teal!40}{.113(.002)}                   
                           &\cellcolor{teal!40}{.435(.003)}&.158(.003)&\cellcolor{teal!40}{.130(.004)}                  
                           &.482(.003)&\cellcolor{teal!40}{.175(.002)}&\cellcolor{teal!40}{.140(.003)}                   
                           &.272(.003)&\cellcolor{teal!40}{.094(.002)}&\cellcolor{teal!40}{.112(.003)}                  
                           &\cellcolor{teal!40}{.297(.003)}&\cellcolor{teal!40}{.070(.003)}&\cellcolor{teal!40}{.087(.003)}                  
                           &\cellcolor{teal!40}{.363(.003)}&\cellcolor{teal!40}{.083(.003)}&.095(.003)                                                            \\ 
\hline

\multirow{4}{*}{\textsc{Law School}} & \multirow{2}{*}{\textit{Gender}}            & w/o \approach                                     
&\cellcolor{teal!40}{.322(.003)}&.122(.004)&\cellcolor{teal!40}{.083(.002)}                  
&.348(.003)&\cellcolor{teal!40}{.132(.003)}&\cellcolor{teal!40}{.092(.002)}                  
&.371(.003)&.154(.003)&\cellcolor{teal!40}{.102(.003)}                   
&\cellcolor{teal!40}{.220(.003)}&\cellcolor{teal!40}{.055(.003)}&.059(.003)                   
&\cellcolor{teal!40}{.250(.002)}&.061(.003)&\cellcolor{teal!40}{.068(.003)}                   
&\cellcolor{teal!40}{.311(.003)}&\cellcolor{teal!40}{.059(.003)}&\cellcolor{teal!40}{.073(.003)}                  
\\ 

                           &                                 & w/ \approach                                      
                           &\cellcolor{teal!40}{.334(.003)}&.128(.003)&\cellcolor{teal!40}{.107(.003)}                  
                           &.356(.003)&\cellcolor{teal!40}{.150(.003)}&\cellcolor{teal!40}{.125(.002)}                  
                           &.398(.002)&.166(.003)&\cellcolor{teal!40}{.133(.003)}                  
                           &\cellcolor{teal!40}{.239(.003)}&\cellcolor{teal!40}{.107(.003)}&.121(.003)                  
                           &\cellcolor{teal!40}{.254(.003)}&.067(.003)&\cellcolor{teal!40}{.095(.002)}                  
                           &\cellcolor{teal!40}{.313(.003)}&\cellcolor{teal!40}{.082(.003)}&\cellcolor{teal!40}{.107(.003)}                                                             \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Race}}           & w/o \approach                                     
                           &.316(.002)&.117(.003)&.084(.003)                  
                           &.342(.003)&\cellcolor{teal!40}{.127(.003)}&\cellcolor{teal!40}{.094(.003)}                   
                           &.386(.002)&\cellcolor{teal!40}{.139(.002)}&\cellcolor{teal!40}{.100(.002)}                  
                           &\cellcolor{teal!40}{.224(.002)}&\cellcolor{teal!40}{.065(.002)}&\cellcolor{teal!40}{.054(.003)}                   
                           &\cellcolor{teal!40}{.256(.003)}&\cellcolor{teal!40}{.071(.004)}&\cellcolor{teal!40}{.065(.002)}                   
                           &\cellcolor{teal!40}{.291(.003)}&\cellcolor{teal!40}{.061(.003)}&\cellcolor{teal!40}{.063(.003)}                   
                           \\ 

                           &                                 & w/ \approach                                       
                           &.322(.003)&.114(.003)&.092(.003)                  
                           &.333(.003)&\cellcolor{teal!40}{.138(.003)}&\cellcolor{teal!40}{.113(.003)}                  
                           &.385(.003)&\cellcolor{teal!40}{.149(.003)}&\cellcolor{teal!40}{.128(.003)}                   
                           &\cellcolor{teal!40}{.251(.003)}&\cellcolor{teal!40}{.104(.003)}&\cellcolor{teal!40}{.111(.003)}                   
                           &\cellcolor{teal!40}{.273(.003)}&\cellcolor{teal!40}{.079(.003)}&\cellcolor{teal!40}{.079(.003)}                   
                           &\cellcolor{teal!40}{.308(.003)}&\cellcolor{teal!40}{.079(.003)}&\cellcolor{teal!40}{.096(.002)}                                                              \\ 
\hline
\multirow{4}{*}{\textsc{Kdd}}       & \multirow{2}{*}{\textit{Gender}}             & w/o \approach                                     
&\cellcolor{teal!40}{.274(.003)}&\cellcolor{teal!40}{.106(.003)}&\cellcolor{teal!40}{.085(.003)}                  
&.288(.003)&\cellcolor{teal!40}{.118(.003)}&\cellcolor{teal!40}{.092(.003)}                   
&\cellcolor{teal!40}{.291(.003)}&\cellcolor{teal!40}{.133(.002)}&\cellcolor{teal!40}{.107(.003)}                   
&.208(.002)&\cellcolor{teal!40}{.064(.002)}&\cellcolor{teal!40}{.061(.002)}                   
&\cellcolor{teal!40}{.228(.003)}&.071(.003)&.076(.003)                   
&\cellcolor{teal!40}{.226(.004)}&\cellcolor{teal!40}{.073(.003)}&\cellcolor{teal!40}{.082(.003)}                                  \\ 

                           &                                  & w/ \approach                                     
                           &\cellcolor{teal!40}{.308(.003)}&\cellcolor{teal!40}{.134(.003)}&\cellcolor{teal!40}{.116(.002)}                   
                           &.309(.002)&\cellcolor{teal!40}{.148(.003)}&\cellcolor{teal!40}{.118(.003)}                   
                           &\cellcolor{teal!40}{.324(.003)}&\cellcolor{teal!40}{.170(.003)}&\cellcolor{teal!40}{.124(.003)}                   
                           &.242(.003)&\cellcolor{teal!40}{.097(.003)}&\cellcolor{teal!40}{.103(.003)}                   
                           &\cellcolor{teal!40}{.246(.002)}&.079(.002)&.102(.004)                   
                           &\cellcolor{teal!40}{.260(.003)}&\cellcolor{teal!40}{.086(.003)}&\cellcolor{teal!40}{.119(.003)}                                                             \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Race}}             & w/o \approach                                      
                           &\cellcolor{teal!40}{.276(.002)}&\cellcolor{teal!40}{.108(.003)}&.094(.003)                   
                           &.292(.002)&.120(.003)&.105(.002)                   
                           &.295(.003)&.137(.003)&.104(.003)                  
                           &\cellcolor{teal!40}{.208(.003)}&\cellcolor{teal!40}{.062(.003)}&\cellcolor{teal!40}{.056(.003)}                  
                           &\cellcolor{teal!40}{.229(.003)}&.068(.003)&\cellcolor{teal!40}{.065(.003)}                  
                           &.227(.003)&\cellcolor{teal!40}{.071(.003)}&\cellcolor{teal!40}{.071(.003)}                                    \\ 

                           &                                  & w/ \approach                                     
                           &\cellcolor{teal!40}{.311(.003)}&\cellcolor{teal!40}{.116(.003)}&.121(.002)                 
                           &.317(.003)&.142(.003)&.119(.003)                  
                           &.332(.003)&.152(.003)&.143(.003)                  
                           &\cellcolor{teal!40}{.238(.003)}&\cellcolor{teal!40}{.097(.003)}&\cellcolor{teal!40}{.104(.003)}                   
                           &\cellcolor{teal!40}{.245(.003)}&.104(.003)&\cellcolor{teal!40}{.111(.003)}                   
                           &.262(.003)&\cellcolor{teal!40}{.092(.003)}&\cellcolor{teal!40}{.120(.003)}                                                           \\ 
\hline
\multirow{4}{*}{\textsc{Dutch}}     & \multirow{2}{*}{\textit{Gender}}            & w/o \approach                                    
&\cellcolor{teal!40}{.282(.002)}&\cellcolor{teal!40}{.111(.002)}&.094(.002)                   
&\cellcolor{teal!40}{.300(.003)}&.127(.003)&\cellcolor{teal!40}{.098(.003)}                   
&\cellcolor{teal!40}{.302(.003)}&.145(.003)&\cellcolor{teal!40}{.108(.003)}                   
&.194(.003)&.076(.003)&\cellcolor{teal!40}{.060(.003)}                   
&.215(.002)&\cellcolor{teal!40}{.080(.003)}&.087(.004)                  
&\cellcolor{teal!40}{.217(.002)}&\cellcolor{teal!40}{.072(.003)}&\cellcolor{teal!40}{.081(.004)}                                      \\ 

                           &                                 & w/ \approach                                     
                           &\cellcolor{teal!40}{.319(.004)}&\cellcolor{teal!40}{.134(.003)}&.100(.003)                   
                           &\cellcolor{teal!40}{.322(.002)}&.149(.003)&\cellcolor{teal!40}{.112(.003)}                 
                           &\cellcolor{teal!40}{.344(.003)}&.162(.003)&\cellcolor{teal!40}{.127(.003)}                   
                           &.235(.003)&.105(.002)&\cellcolor{teal!40}{.112(.003)}                   
                           &.238(.003)&\cellcolor{teal!40}{.095(.003)}&.095(.003)                  
                           &\cellcolor{teal!40}{.252(.003)}&\cellcolor{teal!40}{.087(.003)}&\cellcolor{teal!40}{.102(.003)}                                                            
                           \\
\cline{3-21}
                           & \multirow{2}{*}{\textit{Age}}            & w/o \approach                                    
                           &\cellcolor{teal!40}{.279(.003)}&\cellcolor{teal!40}{.108(.003)}&\cellcolor{teal!40}{.106(.003)}                   
                           &.300(.003)&\cellcolor{teal!40}{.123(.003)}&.110(.002)                   
                           &\cellcolor{teal!40}{.296(.004)}&.136(.002)&\cellcolor{teal!40}{.118(.003)}                   
                           &\cellcolor{teal!40}{.193(.002)}&.055(.003)&.069(.003)                   
                           &\cellcolor{teal!40}{.211(.003)}&.064(.002)&\cellcolor{teal!40}{.081(.003)}                   
                           &\cellcolor{teal!40}{.215(.003)}&\cellcolor{teal!40}{.084(.003)}&\cellcolor{teal!40}{.090(.003)}                                    \\ 

                           &                                 & w/ \approach                                      
                           &\cellcolor{teal!40}{.313(.003)}                   &\cellcolor{teal!40}{.123(.003)}                   &\cellcolor{teal!40}{.131(.003)}                   
                           &.321(.003)                   &\cellcolor{teal!40}{.146(.002)}                   &.124(.003)                   
                           &\cellcolor{teal!40}{.334(.003)}                   &.164(.003)                   &\cellcolor{teal!40}{.144(.003)}                   
                           &\cellcolor{teal!40}{.225(.003)}                   &.102(.002)                   &.116(.003)                   
                           &\cellcolor{teal!40}{.233(.003)}                   &.094(.003)                   &\cellcolor{teal!40}{.103(.003)}                   
                           &\cellcolor{teal!40}{.247(.003)}                   &\cellcolor{teal!40}{.142(.003)}                  &\cellcolor{teal!40}{.122(.003)}                                                            \\ 
\hline
\multirow{6}{*}{\textsc{Credit}}    & \multirow{2}{*}{\textit{Gender}}            & w/o \approach                                      
&\cellcolor{teal!40}{.275(.003)}&.117(.003)&\cellcolor{teal!40}{.101(.002)}                   
&.293(.003)&\cellcolor{red!20}{.129(.003)}&\cellcolor{red!20}{.109(.003)}                   
&\cellcolor{teal!40}{.299(.002)}&\cellcolor{teal!40}{.140(.003)}&.113(.003)                   
&.195(.003)&\cellcolor{teal!40}{.051(.003)}&\cellcolor{teal!40}{.069(.003)}                   
&.214(.003)&.055(.002)&\cellcolor{teal!40}{.077(.003)}                   
&\cellcolor{teal!40}{.217(.003)}&\cellcolor{teal!40}{.063(.003)}&.093(.003)                                      \\ 

                           &                                 & w/ \approach                                       
                           &\cellcolor{teal!40}{.292(.003)}                 &.114(.003)        &\cellcolor{teal!40}{.108(.003)}
                           &.299(.004)                 &\cellcolor{red!20}{.124(.003)}          &\cellcolor{red!20}{.104(.003)}
                           &\cellcolor{teal!40}{.316(.003)}                 &\cellcolor{teal!40}{.157(.003)}        &.111(.003) 
                           &.219(.003)                &\cellcolor{teal!40}{.086(.003)}         &\cellcolor{teal!40}{.101(.003)} 
                           &.215(.003)                &.054(.003)                    &\cellcolor{teal!40}{.088(.003)} 
                           &\cellcolor{teal!40}{.237(.002)}                 &\cellcolor{teal!40}{.069(.003)}        &.093(.003)                                                             \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Marriage}}       & w/o \approach                                      
                           &.286(.003)&\cellcolor{red!20}{.121(.002)}&\cellcolor{teal!40}{.081(.003)}                   
                           &\cellcolor{teal!40}{.303(.003)}&\cellcolor{red!20}{.142(.003)}&\cellcolor{teal!40}{.092(.003)}                   
                           &\cellcolor{teal!40}{.307(.003)}&.153(.003)&\cellcolor{teal!40}{.098(.003)}                   
                           &.245(.003)&.070(.004)&\cellcolor{teal!40}{.061(.002)}                   
                           &.263(.003)&.076(.003)&.073(.003)                   
                           &.267(.003)&\cellcolor{teal!40}{.058(.002)}&.070(.002)                                      \\ 

                           &                                 & w/ \approach                                       
                           &.308(.003)                       &\cellcolor{red!20}{.118(.003)}                  &\cellcolor{teal!40}{.089(.004)} 
                           &\cellcolor{teal!40}{.317(.003)}                       &\cellcolor{red!20}{.135(.002)}                  &\cellcolor{teal!40}{.093(.003)} 
                           &\cellcolor{teal!40}{.324(.003)}                       &.149(.003)                  &\cellcolor{teal!40}{.102(.003)} 
                           &.263(.003)                       &.101(.003)                  &\cellcolor{teal!40}{.092(.003)} 
                           &.261(.003)                       &.073(.003)                  &.067(.003) 
                           &.284(.003)                       &\cellcolor{teal!40}{.079(.003)}                  &.077(.002)                                                          \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Education}}      & w/o \approach                                      
                           &.292(.002)&\cellcolor{teal!40}{.108(.004)}&\cellcolor{teal!40}{.110(.002)}                  
                           &.310(.003)&\cellcolor{teal!40}{.127(.004)}&.136(.003)                  
                           &\cellcolor{teal!40}{.313(.003)}&.139(.003)&.123(.003)                   
                           &\cellcolor{teal!40}{.210(.003)}&.058(.003)&.056(.002)                   
                           &.232(.004)&\cellcolor{teal!40}{.066(.002)}&.065(.003)                   
                           &\cellcolor{teal!40}{.228(.003)}&.081(.002)&.070(.003)                                   \\ 

                           &                                 & w/ \approach                                       
                           &.324(.003)                   &\cellcolor{teal!40}{.136(.003)}                   &\cellcolor{teal!40}{.154(.003)}                   
                           &.327(.003)                   &\cellcolor{teal!40}{.135(.003)}                   &.142(.003)                   
                           &\cellcolor{teal!40}{.343(.003)}                   &.156(.003)                   &.119(.003)                   
                           &\cellcolor{teal!40}{.242(.003)}                   &.102(.003)                   &.097(.003)                   
                           &.245(.003)                   &\cellcolor{teal!40}{.110(.003)}                   &.127(.003)                   
                           &\cellcolor{teal!40}{.263(.003)}                   &.113(.003)                   &.121(.003)                                                              \\ 
\hline
\multirow{4}{*}{\textsc{Crime}}     & \multirow{2}{*}{\textit{Race}}           & w/o \approach                                      
&\cellcolor{teal!40}{.275(.003)}&\cellcolor{red!20}{.132(.003)}&\cellcolor{teal!40}{.081(.003)}                   
&\cellcolor{teal!40}{.293(.002)}&.144(.004)&\cellcolor{teal!40}{.089(.004)}                   
&.292(.002)&\cellcolor{teal!40}{.167(.002)}&\cellcolor{teal!40}{.091(.003)}                   
&\cellcolor{teal!40}{.202(.003)}&\cellcolor{teal!40}{.053(.002)}&\cellcolor{teal!40}{.054(.003)}                   
&.217(.003)&\cellcolor{teal!40}{.058(.003)}&\cellcolor{teal!40}{.066(.002)}                   
&\cellcolor{teal!40}{.225(.003)}&\cellcolor{teal!40}{.065(.003)}&\cellcolor{teal!40}{.064(.003)}                                    \\ 

                           &                                 & w/ \approach                                       
                           &\cellcolor{teal!40}{.307(.003)}&\cellcolor{red!20}{.126(.003)}&\cellcolor{teal!40}{.100(.003)}                   
                           &\cellcolor{teal!40}{.309(.002)}&.150(.002)&\cellcolor{teal!40}{.103(.002)}                   
                           &.331(.003)&\cellcolor{teal!40}{.169(.003)}&\cellcolor{teal!40}{.115(.002)}                   
                           &\cellcolor{teal!40}{.246(.003)}&\cellcolor{teal!40}{.082(.003)}&\cellcolor{teal!40}{.102(.003)}                   
                           &.248(.003)&\cellcolor{teal!40}{.071(.003)}&\cellcolor{teal!40}{.087(.003)}                   
                           &\cellcolor{teal!40}{.269(.003)}&\cellcolor{teal!40}{.082(.004)}&\cellcolor{teal!40}{.097(.002)}                                                               \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Gender}}            & w/o \approach                                      
                           &\cellcolor{teal!40}{.295(.003)}&\cellcolor{teal!40}{.117(.002)}&\cellcolor{teal!40}{.091(.002)}                   
                           &\cellcolor{teal!40}{.314(.003)}&\cellcolor{teal!40}{.129(.003)}&\cellcolor{teal!40}{.102(.003)}                   
                           &\cellcolor{teal!40}{.311(.002)}&\cellcolor{teal!40}{.146(.003)}&.107(.003)                   
                           &\cellcolor{teal!40}{.232(.003)}&\cellcolor{teal!40}{.103(.004)}&.075(.003)                   
                           &\cellcolor{teal!40}{.253(.003)}&\cellcolor{teal!40}{.113(.003)}&\cellcolor{teal!40}{.091(.003)}                   
                           &\cellcolor{teal!40}{.255(.003)}&.059(.003)&\cellcolor{teal!40}{.095(.003)}                                     \\ 

                           &                                 & w/ \approach                                       
                           &\cellcolor{teal!40}{.332(.003)}&\cellcolor{teal!40}{.131(.003)}&\cellcolor{teal!40}{.114(.004)}                   
                           &\cellcolor{teal!40}{.330(.002)}&\cellcolor{teal!40}{.145(.002)}&\cellcolor{teal!40}{.126(.002)}                   
                           &\cellcolor{teal!40}{.352(.002)}&\cellcolor{teal!40}{.168(.003)}&.136(.003)                   
                           &\cellcolor{teal!40}{.271(.003)}&\cellcolor{teal!40}{.114(.003)}&.113(.003)                   
                           &\cellcolor{teal!40}{.278(.002)}&\cellcolor{teal!40}{.117(.002)}&\cellcolor{teal!40}{.113(.003)}                   
                           &\cellcolor{teal!40}{.294(.003)}&.081(.003)&\cellcolor{teal!40}{.119(.003)}                                                              \\ 
\hline 

\multirow{4}{*}{\textsc{German}}    & \multirow{2}{*}{\textit{Gender}}            & w/o \approach                                      
&\cellcolor{teal!40}{.296(.003)}&\cellcolor{teal!40}{.127(.003)}&\cellcolor{teal!40}{.111(.003)}                   
&\cellcolor{teal!40}{.310(.003)}&\cellcolor{teal!40}{.136(.002)}&.120(.003)                   
&\cellcolor{teal!40}{.318(.003)}&.150(.002)&\cellcolor{teal!40}{.131(.003)}                   
&\cellcolor{teal!40}{.206(.002)}&.076(.003)&\cellcolor{teal!40}{.060(.004)}                   
&\cellcolor{teal!40}{.221(.002)}&\cellcolor{teal!40}{.085(.003)}&\cellcolor{teal!40}{.068(.003)}                   
&.223(.003)&\cellcolor{teal!40}{.112(.002)}&\cellcolor{teal!40}{.074(.004)}                                     \\ 

                           &                                 & w/ \approach                                       
                           &\cellcolor{teal!40}{.317(.004)}&\cellcolor{teal!40}{.129(.002)}&\cellcolor{teal!40}{.112(.003)}                  
                           &\cellcolor{teal!40}{.324(.003)}&\cellcolor{teal!40}{.139(.003)}&.145(.003)                   
                           &\cellcolor{teal!40}{.333(.003)}&.150(.003)&\cellcolor{teal!40}{.147(.002)}                   
                           &\cellcolor{teal!40}{.241(.004)}&.097(.003)&\cellcolor{teal!40}{.082(.002)}                  
                           &\cellcolor{teal!40}{.246(.003)}&\cellcolor{teal!40}{.094(.003)}&\cellcolor{teal!40}{.084(.002)}                  
                           &.264(.002)&\cellcolor{teal!40}{.121(.004)}&\cellcolor{teal!40}{.095(.003)}                                                              \\ 
\cline{3-21}
                           & \multirow{2}{*}{\textit{Age}}            & w/o \approach                                     
                           &.276(.003)&\cellcolor{teal!40}{.105(.002)}&\cellcolor{teal!40}{.081(.003)}                  
                           &\cellcolor{teal!40}{.288(.003)}&\cellcolor{teal!40}{.114(.003)}&\cellcolor{teal!40}{.087(.003)}                  
                           &\cellcolor{teal!40}{.296(.003)}&\cellcolor{teal!40}{.124(.003)}&.096(.003)                   
                           &\cellcolor{teal!40}{.223(.003)}&\cellcolor{teal!40}{.085(.003)}&\cellcolor{teal!40}{.080(.003)}                   
                           &.245(.003)&\cellcolor{teal!40}{.096(.002)}&.069(.003)                  
                           &\cellcolor{teal!40}{.242(.003)}&\cellcolor{teal!40}{.087(.002)}&\cellcolor{teal!40}{.075(.004)}                                      \\ 

                           &                                 & w/ \approach                                   &.284(.003)&\cellcolor{teal!40}{.142(.004)}&\cellcolor{teal!40}{.113(.003)}                   
                        &\cellcolor{teal!40}{.311(.003)}&\cellcolor{teal!40}{.154(.003)}&\cellcolor{teal!40}{.127(.003)}                  
                        &\cellcolor{teal!40}{.329(.003)}&\cellcolor{teal!40}{.156(.003)}&.134(.003)                   
                        &\cellcolor{teal!40}{.258(.003)}&\cellcolor{teal!40}{.124(.003)}&\cellcolor{teal!40}{.129(.003)}                   
                        &.259(.003)&\cellcolor{teal!40}{.125(.003)}&.111(.003)                   
                        &\cellcolor{teal!40}{.280(.003)}&\cellcolor{teal!40}{.103(.003)}&\cellcolor{teal!40}{.114(.003)}                                                           \\
\hline
%\bottomrule

\end{tabular}
\end{adjustbox}
\arrayrulecolor{black}
\vspace{-0.4cm}
\end{table*}

==> Table/rq2-new1.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table*}[t!]
\caption{Comparing \approach~with \texttt{FairRF}, which ranks non-sensitive attributes with respect to the sensitive one based on correlation analysis, over all cases using the mean (standard deviation) of all fairness metrics under 10 runs. $f_c$ denotes the direct and most causally relevant non-sensitive feature to the concerned sensitive one. The other format is the same as Table~\ref{tb:rq1}.}

\label{tb:rq2}
\setlength{\tabcolsep}{.7mm}
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{llll|rrr|rrr|rrr|rrr|rrr|rrr} 
\toprule
\multirow{2}{*}{\textbf{Dataset}}   & \multirow{2}{*}{\textbf{$f_s$}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Approach}}}   & \multirow{2}{*}{\textbf{$f_c$}} & \multicolumn{3}{c|}{\texttt{ADF}}                                                       & \multicolumn{3}{c|}{\texttt{EIDIG}}                                                     & \multicolumn{3}{c|}{\texttt{NeuronFair}}                                                & \multicolumn{3}{c|}{\texttt{SG}}                                                        & \multicolumn{3}{c|}{\texttt{ExpGA}}                                                     & \multicolumn{3}{c}{\texttt{BREAM}}                                                      \\ 
\cline{5-22}
                           &           &                      & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l|}{SPD} & \multicolumn{1}{l}{IDI ratio} & \multicolumn{1}{l}{EOD} & \multicolumn{1}{l}{SPD}                                            \\ 
\midrule
\multirow{6}{*}{\textsc{Adult}}     & \multirow{2}{*}{\textit{Gender}}            &\approach &\textit{Relationship} 
                           &.301(.003)                   &\cellcolor{teal!40}{.142(.003)}                   &\cellcolor{teal!40}{.103(.003)}       
                           &\cellcolor{teal!40}{.316(.003)}                   &\cellcolor{teal!40}{.169(.003)}                   &.120(.003)                  
                           &\cellcolor{teal!40}{.365(.004)}                   &.154(.002)                   &\cellcolor{teal!40}{.137(.003)}                   
                           &\cellcolor{teal!40}{.262(.003)}                   &\cellcolor{teal!40}{.127(.003)}                   &.116(.003)                  
                           &\cellcolor{teal!40}{.274(.003)}                   &\cellcolor{teal!40}{.092(.003)}                   &.104(.002)                   
                           &.284(.003)                   &\cellcolor{teal!40}{.109(.003)}                   &\cellcolor{teal!40}{.121(.003)}                                  \\ 

                           &                                 & \texttt{FairRF} &\textit{Workclass}                 
                           &.293(.003)                    &\cellcolor{teal!40}{.109(.003)}                    &\cellcolor{teal!40}{.085(.003)}                   
                           &\cellcolor{teal!40}{.283(.003)}                    &\cellcolor{teal!40}{.126(.003)}                    &.078(.004)                   
                           &\cellcolor{teal!40}{.339(.002)}                    &.143(.002)                    &\cellcolor{teal!40}{.107(.001)}                           
                           &\cellcolor{teal!40}{.222(.003)}                    &\cellcolor{teal!40}{.067(.003)}                    &.085(.002)                    
                           &\cellcolor{teal!40}{.257(.004)}                    &\cellcolor{teal!40}{.065(.003)}                    &.102(.003)                   
                           &.263(.002)                    &\cellcolor{teal!40}{.075(.003)}                    &\cellcolor{teal!40}{.109(.003)}                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Race}}   &\approach &\textit{Native-country}         
                           &.382(.003)                 &.113(.003)                   &\cellcolor{teal!40}{.132(.003)}     
                           &\cellcolor{teal!40}{.396(.003)}                 &\cellcolor{teal!40}{.131(.003)}                  &\cellcolor{teal!40}{.145(.003)}                  
                           &\cellcolor{teal!40}{.429(.003)}                 &\cellcolor{teal!40}{.154(.002)}                   &\cellcolor{teal!40}{.155(.003)}   
                           &.249(.003)                 &\cellcolor{teal!40}{.102(.003)}                   &\cellcolor{teal!40}{.116(.003)}   
                           &\cellcolor{teal!40}{.251(.003)}                 &.079(.003)                   &.079(.001)   
                           &\cellcolor{teal!40}{.316(.003)}                 &\cellcolor{teal!40}{.086(.002)}                   &\cellcolor{teal!40}{.097(.003)}                    \\ 

                           &                         & \texttt{FairRF} &\textit{Education}             
                           &.377(.003)                    &.105(.002)                    &\cellcolor{teal!40}{.068(.002)}                   
                           &\cellcolor{teal!40}{.341(.002)}                    &\cellcolor{teal!40}{.109(.003)}                    &\cellcolor{teal!40}{.134(.002)}                    
                           &\cellcolor{teal!40}{.341(.003)}                    &\cellcolor{teal!40}{.148(.002)}                    &\cellcolor{teal!40}{.139(.003)}                           
                           &.165(.003)                    &\cellcolor{teal!40}{.057(.003)}                    &\cellcolor{teal!40}{.073(.003)}                    
                           &\cellcolor{teal!40}{.217(.003)}                    &.075(.003)                    &.072(.003)                   
                           &\cellcolor{teal!40}{.307(.003)}                    &\cellcolor{teal!40}{.074(.003)}                    &\cellcolor{teal!40}{.092(.003)}                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Age}}     &\approach &\textit{Marital-status}         
                           &.353(.003)                    &.111(.002)                    &.117(.003)                    
                           &.357(.002)                    &.113(.004)                    &.104(.003)                    
                           &.388(.003)                    &.209(.004)                    &.122(.003)                          
                           &.251(.003)                    &.122(.003)                    &.098(.003)                   
                           &.274(.003)                    &.056(.003)                    &.069(.003)                   
                           &.308(.003)                    &.063(.002)                    &.074(.003)                     \\ 

                           &                        & \texttt{FairRF} &\textit{Marital-status}        
                           &.353(.003)                    &.111(.002)                    &.117(.003)                    
                           &.357(.002)                    &.113(.004)                    &.104(.003)                    
                           &.388(.003)                    &.209(.004)                    &.122(.003)                          
                           &.251(.002)                    &.122(.003)                    &.098(.003)                   
                           &.274(.003)                    &.056(.003)                    &.069(.003)                   
                           &.308(.003)                    &.063(.002)                    &.074(.003)                     \\ 
\hline
\multirow{4}{*}{\textsc{Compas}}    & \multirow{2}{*}{\textit{Gender}}    &\approach &\textit{Previous Convictions}           
&\cellcolor{teal!40}{.386(.003)}                   &.144(.003)                   &\cellcolor{teal!40}{.130(.002)}                   
&\cellcolor{teal!40}{.394(.003)}                   &\cellcolor{teal!40}{.157(.003)}                   &\cellcolor{teal!40}{.124(.003)}                   
&\cellcolor{teal!40}{.419(.003)}                   &.163(.003)                   &\cellcolor{teal!40}{.153(.003)}                   
&\cellcolor{teal!40}{.247(.003)}                   &\cellcolor{teal!40}{.103(.002)}                   &\cellcolor{teal!40}{.094(.003)}                  
&.272(.003)                   &.092(.003)                   &.105(.003)                   
&\cellcolor{teal!40}{.335(.003)}                   &\cellcolor{teal!40}{.110(.003)}                   &\cellcolor{red!20}{.126(.003)}                     \\ 

                           &                        & \texttt{FairRF} &\textit{Decile-text}           
                           &\cellcolor{teal!40}{.362(.003)}&.115(.003)&\cellcolor{teal!40}{.077(.003)}                   
                           &\cellcolor{teal!40}{.377(.003)}&\cellcolor{teal!40}{.096(.003)}&\cellcolor{teal!40}{.101(.003)}                    
                           &\cellcolor{teal!40}{.383(.002)}&.157(.003)&\cellcolor{teal!40}{.111(.002)}       
                           &\cellcolor{teal!40}{.211(.003)}&\cellcolor{teal!40}{.056(.003)}&\cellcolor{teal!40}{.068(.003)}                    
                           &.249(.003)&.064(.003)&.173(.003)                    
                           &\cellcolor{teal!40}{.291(.003)}&\cellcolor{teal!40}{.106(.003)}&\cellcolor{red!20}{.132(.002)}                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Race}}   &\approach &\textit{Compas-score}         
                           &\cellcolor{teal!40}{.426(.003)}&\cellcolor{teal!40}{.138(.002)}&\cellcolor{teal!40}{.113(.002)}                   
                           &\cellcolor{teal!40}{.435(.003)}&.158(.003)&.130(.004)                  
                           &\cellcolor{teal!40}{.482(.003)}&\cellcolor{teal!40}{.175(.002)}&.140(.003)                   
                           &\cellcolor{teal!40}{.272(.003)}&\cellcolor{teal!40}{.094(.002)}&.112(.003)                   
                           &.297(.003)&\cellcolor{teal!40}{.070(.003)}&\cellcolor{teal!40}{.087(.003)}                  
                           &\cellcolor{teal!40}{.363(.003)}&.083(.003)&\cellcolor{teal!40}{.095(.003)}                    \\ 

                           &                         & \texttt{FairRF} &\textit{Decile-text}            
                           &\cellcolor{teal!40}{.405(.003)}&\cellcolor{teal!40}{.112(.003)}&\cellcolor{teal!40}{.104(.003)}                    
                           &\cellcolor{teal!40}{.411(.002)}&.137(.003)&.121(.003)                    
                           &\cellcolor{teal!40}{.432(.003)}&\cellcolor{teal!40}{.142(.003)}&.125(.003)
                           &\cellcolor{teal!40}{.227(.002)}&\cellcolor{teal!40}{.064(.003)}&.081(.002)                    
                           &.263(.003)&\cellcolor{teal!40}{.066(.002)}&\cellcolor{teal!40}{.069(.003)}                    
                           &\cellcolor{teal!40}{.323(.003)}&.079(.004)&\cellcolor{teal!40}{.083(.003)}                     \\ 
\hline
\multirow{4}{*}{\textsc{Law School}} & \multirow{2}{*}{\textit{Gender}}     &\approach &\textit{Lsat}          
&\cellcolor{teal!40}{.334(.003)}&\cellcolor{teal!40}{.128(.003)}&\cellcolor{teal!40}{.107(.003)}                   
&.356(.003)&\cellcolor{teal!40}{.150(.003)}&\cellcolor{teal!40}{.125(.002)}                   
&.398(.002)&.166(.003)&\cellcolor{teal!40}{.133(.003)}                   
&.239(.003)&\cellcolor{teal!40}{.107(.003)}&.121(.003)                   
&\cellcolor{teal!40}{.254(.003)}&.067(.003)&.095(.002)                   
&\cellcolor{teal!40}{.313(.003)}&\cellcolor{teal!40}{.082(.003)}&\cellcolor{teal!40}{.107(.003)}                    \\ 

                           &                         & \texttt{FairRF} &\textit{Decile1b}             
                           &\cellcolor{teal!40}{.301(.003)}&\cellcolor{teal!40}{.094(.003)}&\cellcolor{teal!40}{.086(.003)}                   
                           &.322(.004)&\cellcolor{teal!40}{.128(.003)}&\cellcolor{teal!40}{.104(.002)}                   
                           &.352(.003)&.142(.004)&\cellcolor{teal!40}{.127(.003)}                           
                           &.198(.002)&\cellcolor{teal!40}{.062(.003)}&.117(.005)                    
                           &\cellcolor{teal!40}{.216(.003)}&.072(.003)&.083(.004)                   
                           &\cellcolor{teal!40}{.247(.002)}&\cellcolor{teal!40}{.074(.004)}&\cellcolor{teal!40}{.093(.003)}                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Race}}    &\approach &\textit{Lsat}                 
                           &\cellcolor{teal!40}{.322(.003)}                   &\cellcolor{teal!40}{.114(.003)}                   &.092(.003)                   
                           &.333(.003)                   &.138(.003)                   &\cellcolor{teal!40}{.113(.003)}                   
                           &.385(.003)                   &\cellcolor{teal!40}{.149(.003)}                   &.128(.003)                   
                           &\cellcolor{teal!40}{.251(.003)}                   &\cellcolor{teal!40}{.102(.002)}                   &\cellcolor{teal!40}{.111(.003)}                   
                           &\cellcolor{teal!40}{.273(.003)}                   &\cellcolor{red!20}{.079(.003)}                   &\cellcolor{teal!40}{.079(.003)}                   
                           &\cellcolor{teal!40}{.308(.003)}                   &\cellcolor{red!20}{.079(.003)}                   &.096(.002)                    \\ 

                           &                         & \texttt{FairRF} &\textit{Delice3}      
                           &\cellcolor{teal!40}{.319(.003)}                    &\cellcolor{teal!40}{.105(.003)}                    &.090(.003)     
                           &.325(.003)                    &.136(.003)                    &\cellcolor{teal!40}{.107(.002)}      
                           &.367(.003)                    &\cellcolor{teal!40}{.141(.003)}                    &.113(.002)     
                           &\cellcolor{teal!40}{.232(.003)}                    &\cellcolor{teal!40}{.081(.002)}                    &\cellcolor{teal!40}{.077(.003)}       
                           &\cellcolor{teal!40}{.267(.003)}                    &\cellcolor{red!20}{.108(.002)}                    &\cellcolor{teal!40}{.071(.003)}      
                           &\cellcolor{teal!40}{.302(.003)}                    &\cellcolor{red!20}{.116(.003)}                    &.085(.003)                     \\ 
\hline
\multirow{4}{*}{\textsc{Kdd}}       & \multirow{2}{*}{\textit{Gender}}     &\approach &\textit{Occupation}      
                           &\cellcolor{teal!40}{.308(.003)}                   &\cellcolor{teal!40}{.134(.003)}                   &.116(.002)                   
                           &\cellcolor{teal!40}{.309(.002)}                   &.148(.003)                   &.118(.003)                   
                           &\cellcolor{teal!40}{.324(.003)}                   &\cellcolor{teal!40}{.170(.003)}                   &\cellcolor{teal!40}{.124(.003)}                   
                           &\cellcolor{teal!40}{.251(.003)}                   &\cellcolor{teal!40}{.097(.002)}                   &.103(.003)                   
                           &\cellcolor{teal!40}{.246(.002)}                   &\cellcolor{teal!40}{.079(.002)}                   &\cellcolor{teal!40}{.102(.004)}                   
                           &.260(.003)                   &.086(.003)                   &\cellcolor{teal!40}{.119(.003)}                   \\ 

                           &                        & \texttt{FairRF} &\textit{Housing}        
                           &\cellcolor{teal!40}{.276(.003)}                    &\cellcolor{teal!40}{.114(.003)}                    &.114(.003)         
                           &\cellcolor{teal!40}{.289(.003)}                    &.124(.002)                    &.097(.003)         
                           &\cellcolor{teal!40}{.318(.002)}                    &\cellcolor{teal!40}{.152(.003)}                    &\cellcolor{teal!40}{.111(.003)}        
                           &\cellcolor{teal!40}{.218(.003)}                    &\cellcolor{teal!40}{.071(.003)}                    &.087(.003)        
                           &\cellcolor{teal!40}{.227(.003)}                    &\cellcolor{teal!40}{.076(.003)}                    &\cellcolor{teal!40}{.093(.003)}        
                           &.253(.002)                    &.077(.003)                    &\cellcolor{teal!40}{.108(.003)}                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Race}}    &\approach &\textit{Tax-filer-stat}    
                           &\cellcolor{teal!40}{.311(.003)}&.116(.003)&.121(.002)                 
                           &\cellcolor{teal!40}{.317(.003)}&\cellcolor{teal!40}{.142(.003)}&\cellcolor{teal!40}{.119(.003)}                  
                           &\cellcolor{teal!40}{.332(.003)}&\cellcolor{teal!40}{.152(.003)}&\cellcolor{teal!40}{.143(.003)}                  
                           &.242(.003)&\cellcolor{teal!40}{.097(.003)}&.103(.003)                   
                           &\cellcolor{teal!40}{.245(.003)}&.104(.003)&\cellcolor{teal!40}{.111(.003)}                   
                           &\cellcolor{teal!40}{.262(.003)}&\cellcolor{teal!40}{.092(.003)}&.120(.003)                   \\ 

                           &                         & \texttt{FairRF} &\textit{Marital-status}   
                           &\cellcolor{teal!40}{.291(.002)}&.112(.003)&.087(.003)             
                           &\cellcolor{teal!40}{.304(.003)}&\cellcolor{teal!40}{.120(.002)}&\cellcolor{teal!40}{.089(.003)}             
                           &\cellcolor{teal!40}{.314(.003)}&\cellcolor{teal!40}{.132(.002)}&\cellcolor{teal!40}{.114(.003)} 
                           &.221(.002)&\cellcolor{teal!40}{.065(.002)}&.071(.003)      
                           &\cellcolor{teal!40}{.237(.004)}&.071(.003)&\cellcolor{teal!40}{.077(.004)}     
                           &\cellcolor{teal!40}{.243(.003)}&\cellcolor{teal!40}{.069(.003)}&.066(.002)                     \\ 
\hline
\multirow{4}{*}{\textsc{Dutch}}     & \multirow{2}{*}{\textit{Gender}}     &\approach &\textit{Cur\_eco\_activity}  
                           &.319(.004)                   &.134(.003)                   &.100(.003)                   
                           &.322(.002)                   &.149(.003)                   &.112(.003)                   
                           &.344(.003)                   &.162(.003)                   &.127(.003)                   
                           &.233(.003)                   &.089(.002)                   &.091(.002)                   
                           &.238(.003)                   &.095(.003)                   &.095(.003)                  
                           &.252(.003)                   &.087(.003)                   &.102(.003)                    \\ 

                           &                        & \texttt{FairRF} &\textit{Cur\_eco\_activity}   
                           &.319(.004)                   &.134(.003)                   &.100(.003)                   
                           &.322(.002)                   &.149(.003)                   &.112(.003)                   
                           &.344(.003)                   &.162(.003)                   &.127(.003)                   
                           &.233(.003)                   &.089(.002)                   &.091(.002)                   
                           &.238(.003)                   &.095(.003)                   &.095(.003)                  
                           &.252(.003)                   &.087(.003)                   &.102(.003)                     \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Age}}     &\approach &\textit{Economic\_status}      
                           &\cellcolor{teal!40}{.313(.003)}                   &\cellcolor{teal!40}{.123(.003)}                   &.131(.003)                   
                           &\cellcolor{teal!40}{.321(.003)}                   &\cellcolor{teal!40}{.146(.002)}                   &\cellcolor{teal!40}{.124(.003)}                   
                           &.334(.003)                   &.164(.003)                   &.144(.003)                   
                           &\cellcolor{teal!40}{.235(.003)}                   &\cellcolor{teal!40}{.105(.003)}                   &.112(.003)                   
                           &\cellcolor{teal!40}{.233(.003)}                   &.094(.003)                   &\cellcolor{teal!40}{.103(.003)}                   
                           &\cellcolor{teal!40}{.247(.003)}                   &.142(.003)                   &\cellcolor{teal!40}{.122(.003)}                    \\ 

                           &                         & \texttt{FairRF} &\textit{Edu\_level}        
                           &\cellcolor{teal!40}{.297(.003)}                    &\cellcolor{teal!40}{.102(.003)}                    &.110(.003)                
                           &\cellcolor{teal!40}{.301(.003)}                    &\cellcolor{teal!40}{.129(.003)}                    &\cellcolor{teal!40}{.113(.003)}               
                           &.314(.003)                    &.131(.003)                    &.117(.003)             
                           &\cellcolor{teal!40}{.212(.002)}                    &\cellcolor{teal!40}{.068(.002)}                    &.088(.003)         
                           &\cellcolor{teal!40}{.223(.003)}                    &.068(.003)                    &\cellcolor{teal!40}{.092(.003)}          
                           &\cellcolor{teal!40}{.235(.002)}                    &.139(.001)                   &\cellcolor{teal!40}{.101(.003)}                     \\
\hline  
\multirow{6}{*}{\textsc{Credit}}    & \multirow{2}{*}{\textit{Gender}}            &\approach &\textit{Pay\_amt3}             
                           &.292(.003)                 &.114(.003)                    &.108(.003)
                           &.299(.004)                 &.124(.003)                    &.104(.003)
                           &.316(.003)                 &.157(.003)                    &.111(.003) 
                           &.219(.003)                 &.086(.003)                    &.101(.003) 
                           &.215(.003)                 &.054(.003)                    &.088(.003) 
                           &.237(.002)                 &.069(.003)                    &.093(.003)                                   \\ 

                           &                                 & \texttt{FairRF} &\textit{Pay\_amt3}  
                           &.292(.003)                 &.114(.003)                    &.108(.003)
                           &.299(.004)                 &.124(.003)                    &.104(.003)
                           &.316(.003)                 &.157(.003)                    &.111(.003) 
                           &.219(.003)                 &.086(.003)                    &.101(.003) 
                           &.215(.003)                 &.054(.003)                    &.088(.003) 
                           &.237(.002)                 &.069(.003)                    &.093(.003) 
                                                            \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Marriage}}       &\approach &\textit{Pay\_amt1}   
                           &.308(.003)                       &.118(.003)                  &.089(.004) 
                           &.317(.003)                       &.135(.002)                  &.093(.003) 
                           &.324(.003)                       &.149(.003)                  &.102(.003) 
                           &.263(.003)                       &.101(.003)                  &.092(.003) 
                           &.261(.003)                       &.073(.003)                  &.067(.003) 
                           &.284(.003)                       &.079(.003)                  &.077(.002) 
                                     \\ 

                           &                                 & \texttt{FairRF} &\textit{Pay\_amt1}  
                           &.308(.003)                       &.118(.003)                  &.089(.004) 
                           &.317(.003)                       &.135(.002)                  &.093(.003) 
                           &.324(.003)                       &.149(.003)                  &.102(.003) 
                           &.263(.003)                       &.101(.003)                  &.092(.003) 
                           &.261(.003)                       &.073(.003)                  &.067(.003) 
                           &.284(.003)                       &.079(.003)                  &.077(.002)
                                                          \\ 
\cline{3-22}
                           & \multirow{2}{*}{\textit{Education}}      &\approach &\textit{Pay\_amt1}                    
                           &.324(.003)                   &\cellcolor{teal!40}{.136(.003)}                   &\cellcolor{teal!40}{.154(.003)}                   
                           &\cellcolor{teal!40}{.327(.003)}                   &.135(.003)                   &\cellcolor{teal!40}{.142(.003)}                   
                           &.343(.003)                   &\cellcolor{teal!40}{.156(.003)}                   &\cellcolor{teal!40}{.119(.003)}                   
                           &\cellcolor{teal!40}{.242(.003)}                   &\cellcolor{teal!40}{.102(.003)}                   &\cellcolor{teal!40}{.097(.003)}                   
                           &\cellcolor{teal!40}{.245(.003)}                   &.110(.003)                   &.127(.003)                   
                           &\cellcolor{teal!40}{.263(.003)}                   &.113(.003)                   &\cellcolor{teal!40}{.121(.003)}                                                              \\                                

                           &                                 & \texttt{FairRF} &\textit{BILL\_AMT3}   
                           &.310(.003)                  &\cellcolor{teal!40}{.109(.004)}                 &\cellcolor{teal!40}{.104(.004)} 
                           &\cellcolor{teal!40}{.311(.003)}                  &.128(.003)                 &\cellcolor{teal!40}{.109(.003)} 
                           &.331(.003)                  &\cellcolor{teal!40}{.142(.003)}                 &\cellcolor{teal!40}{.114(.003)} 
                           &\cellcolor{teal!40}{.228(.003)}                  &\cellcolor{teal!40}{.063(.003)}                 &\cellcolor{teal!40}{.069(.002)} 
                           &\cellcolor{teal!40}{.232(.003)}                  &.068(.003)                 &.072(.003) 
                           &\cellcolor{teal!40}{.248(.003)}                  &.082(.002)                 &\cellcolor{teal!40}{.084(.003)}
 \\ 
\hline

\multirow{4}{*}{\textsc{Crime}}  & \multirow{2}{*}{\textit{Race}} &\approach &\textit{Score\_text}    
                           &.307(.003)                   &.126(.003)                   &.100(.003)                   
                           &.309(.002)                   &.150(.002)                   &.103(.002)                   
                           &.331(.003)                   &.169(.003)                   &.115(.002)                   
                           &.246(.003)                   &.082(.003)                   &.102(.003)                   
                           &.248(.003)                   &.071(.003)                   &.087(.003)                   
                           &.269(.003)                   &.082(.004)                   &.097(.002)   \\ 

                        &                       & \texttt{FairRF} &\textit{Score\_text}    
                           &.307(.003)                   &.126(.003)                   &.100(.003)                   
                           &.309(.002)                   &.150(.002)                   &.103(.002)                   
                           &.331(.003)                   &.169(.003)                   &.115(.002)                   
                           &.246(.003)                   &.082(.003)                   &.102(.003)                   
                           &.248(.003)                   &.071(.003)                   &.087(.003)                   
                           &.269(.003)                   &.082(.004)                   &.097(.002)   \\ 
\cline{3-22}
                        & \multirow{2}{*}{\textit{Gender}}  &\approach &\textit{Priors\_count}  
                          &\cellcolor{teal!40}{.332(.003)}                   &\cellcolor{teal!40}{.131(.003)}                   &.114(.004)                   
                          &\cellcolor{teal!40}{.330(.002)}                   &\cellcolor{teal!40}{.145(.002)}                   &\cellcolor{teal!40}{.126(.002)}                   
                          &\cellcolor{teal!40}{.352(.002)}                   &.168(.003)                   &.136(.003)                   
                          &\cellcolor{teal!40}{.271(.003)}                   &\cellcolor{teal!40}{.114(.003)}                   &.102(.003)                   
                          &.278(.002)                   &\cellcolor{teal!40}{.117(.002)}                   &\cellcolor{teal!40}{.113(.003)}                  
                          &\cellcolor{teal!40}{.294(.003)}                   &.081(.003)                   &\cellcolor{teal!40}{.119(.003)}  \\ 

                        &                       & \texttt{FairRF} &\textit{V\_score\_text} 
                          &\cellcolor{teal!40}{.311(.003)}                &\cellcolor{teal!40}{.117(.004)}                &.104(.003) 
                          &\cellcolor{teal!40}{.312(.003)}                &\cellcolor{teal!40}{.121(.003)}                &\cellcolor{teal!40}{.105(.002)} 
                          &\cellcolor{teal!40}{.336(.003)}                &.134(.003)                &.112(.002) 
                          &\cellcolor{teal!40}{.244(.004)}                &\cellcolor{teal!40}{.103(.003)}                &.091(.003) 
                          &.252(.004)                &\cellcolor{teal!40}{.104(.002)}                &\cellcolor{teal!40}{.097(.003)} 
                          &\cellcolor{teal!40}{.278(.003)}                &.083(.003)                &\cellcolor{teal!40}{.107(.003)}  \\ 
\hline
\multirow{4}{*}{\textsc{German}} & \multirow{2}{*}{\textit{Gender}}  &\approach &\textit{Credit-amount}  
                           &.317(.004)                   &.129(.002)                  &.112(.003)                 
                           &.324(.003)                   &.139(.003)                  &.145(.003)                   
                           &.333(.003)                   &.150(.003)                  &.147(.002)                   
                           &.241(.004)                   &.097(.003)                  &.082(.002)                  
                           &.246(.003)                   &.094(.003)                  &.084(.002)                  
                           &.264(.002)                   &.121(.004)                  &.095(.003) \\ 

                        &                       & \texttt{FairRF} &\textit{Credit-amount}  
                           &.317(.004)                   &.129(.002)                  &.112(.003)                 
                           &.324(.003)                   &.139(.003)                  &.145(.003)                   
                           &.333(.003)                   &.150(.003)                  &.147(.002)                   
                           &.241(.004)                   &.097(.003)                  &.082(.002)                  
                           &.246(.003)                   &.094(.003)                  &.084(.002)                  
                           &.264(.002)                   &.121(.004)                  &.095(.003)  \\ 
\cline{3-22}
                        & \multirow{2}{*}{\textit{Age}}  &\approach &\textit{Existing-credits}       
                        &.284(.003)&\cellcolor{teal!40}{.142(.004)}&\cellcolor{teal!40}{.113(.003)}                   
                        &\cellcolor{teal!40}{.311(.003)}&.154(.003)&\cellcolor{teal!40}{.127(.003)}                  
                        &\cellcolor{teal!40}{.329(.003)}&.156(.003)&\cellcolor{teal!40}{.134(.003)}                   
                        &.258(.003)&\cellcolor{teal!40}{.124(.003)}&\cellcolor{teal!40}{.129(.003)}                   
                        &\cellcolor{teal!40}{.259(.003)}&\cellcolor{teal!40}{.125(.003)}&\cellcolor{teal!40}{.111(.003)}                   
                        &\cellcolor{teal!40}{.280(.003)}&.103(.003)&\cellcolor{teal!40}{.114(.003)} \\ 
                        &                       & \texttt{FairRF} &\textit{Duration}       
                        &.269(.003)&\cellcolor{teal!40}{.126(.003)}&\cellcolor{teal!40}{.084(.003)} 
                        &\cellcolor{teal!40}{.305(.003)}&.128(.002)&\cellcolor{teal!40}{.094(.002)} 
                        &\cellcolor{teal!40}{.317(.003)}&.143(.002)&\cellcolor{teal!40}{.108(.003)} 
                        &.247(.003)&\cellcolor{teal!40}{.083(.003)}&\cellcolor{teal!40}{.078(.002)} 
                        &\cellcolor{teal!40}{.246(.003)}&\cellcolor{teal!40}{.094(.003)}&\cellcolor{teal!40}{.087(.002)} 
                        &\cellcolor{teal!40}{.269(.003)}&.081(.003)&\cellcolor{teal!40}{.083(.003)}  \\
\hline
%\bottomrule

\end{tabular}
\end{adjustbox}
\arrayrulecolor{black}
\vspace{-0.4cm}
\end{table*}

==> Table/rq4-new1.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}[t!]
\caption{Testing the retrained DNN improved by \approach~against before retraining, without \approach, and \texttt{FairRF} over 5 retraining runs $\times$ 10 testing runs (i.e., $A-B$ where $A$ and $B$ are the metric values of testing the retrained DNN by other and \approach, respectively). All retrained samples are generated with the best generator under an approach. Positive numbers imply \approach~improves more. \setlength{\fboxsep}{1.5pt}\colorbox{teal!40}{green cells} mean the improvement is statistically significant.}

\label{tb:rq4}
\setlength{\tabcolsep}{.5mm}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ll|lll|lll|lll} 
\toprule

\multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{$f_s$}&\multicolumn{3}{c|}{IDI ratio (\approach~vs.)}&\multicolumn{3}{c|}{EOD (\approach~vs.)}&\multicolumn{3}{c}{SPD (\approach~vs.)}\\

\cline{3-11}

&&Before&w/o&\texttt{FairRF}&Before&w/o&\texttt{FairRF}&Before&w/o&\texttt{FairRF}\\

\midrule

\multirow{3}{*}{\textsc{Adult}}&\textit{Gender}
&\cellcolor{teal!40}{.214(.002)}&.033(.003)&.046(.003)
&\cellcolor{teal!40}{.084(.002)}&\cellcolor{teal!40}{.017(.002)}&\cellcolor{teal!40}{.021(.002)}
&\cellcolor{teal!40}{.041(.002)}&\cellcolor{teal!40}{.012(.002)}&\cellcolor{teal!40}{.013(.002)}\\

&\textit{Race}&.248(.003)&\cellcolor{teal!40}{.042(.003)}&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.078(.002)}&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.029(.002)}&\cellcolor{teal!40}{.074(.002)}&\cellcolor{teal!40}{.014(.002)}&\cellcolor{teal!40}{.017(.002)}\\

&\textit{Age}&\cellcolor{teal!40}{.225(.003)}&\cellcolor{teal!40}{.036(.003)}&\cellcolor{teal!40}{.021(.006)}&\cellcolor{teal!40}{.091(.002)}&\cellcolor{teal!40}{.016(.002)}&\cellcolor{teal!40}{.013(.005)}&\cellcolor{teal!40}{.066(.002)}&\cellcolor{teal!40}{.008(.001)}&\cellcolor{teal!40}{.011(.005)}\\

\hline


\multirow{2}{*}{\textsc{Compas}}&\textit{Gender}&\cellcolor{teal!40}{.257(.003)}&\cellcolor{teal!40}{.038(.003)}&\cellcolor{teal!40}{.044(.004)}&\cellcolor{teal!40}{.081(.002)}&\cellcolor{teal!40}{.018(.002)}&\cellcolor{teal!40}{.026(.002)}&\cellcolor{teal!40}{.051(.002)}&.014(.002)&.011(.002)\\

&\textit{Race}&\cellcolor{teal!40}{.290(.003)}&\cellcolor{teal!40}{.036(.004)}&\cellcolor{teal!40}{.051(.003)}&.092(.002)&.021(.003)&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.081(.002)}&\cellcolor{teal!40}{.012(.002)}&.010(.001)\\

\hline

\multirow{2}{*}{\textsc{Law School}}&\textit{Gender}&\cellcolor{teal!40}{.235(.003)}&\cellcolor{teal!40}{.036(.003)}&.042(.003)&.088(.002)&\cellcolor{teal!40}{.019(.005)}&\cellcolor{teal!40}{.019(.001)}&\cellcolor{teal!40}{.069(.002)}&\cellcolor{teal!40}{.013(.002)}&.008(.001)\\

&\textit{Race}&\cellcolor{teal!40}{.228(.003)}&.039(.003)&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.077(.003)}&\cellcolor{teal!40}{.024(.003)}&.023(.002)&.063(.002)&\cellcolor{teal!40}{.015(.002)}&.011(.001)\\

\hline


\multirow{2}{*}{\textsc{KDD}}&\textit{Gender}&.184(.003)&\cellcolor{teal!40}{.027(.003)}&\cellcolor{teal!40}{.037(.002)}&\cellcolor{teal!40}{.082(.002)}&\cellcolor{teal!40}{.016(.003)}&.021(.003)&.061(.002)&\cellcolor{teal!40}{.010(.002)}&.012(.004)\\

&\textit{Race}&.192(.003)&\cellcolor{teal!40}{.034(.005)}&\cellcolor{teal!40}{.052(.003)}&.073(.002)&\cellcolor{teal!40}{.020(.003)}&.017(.002)&\cellcolor{teal!40}{.064(.002)}&\cellcolor{teal!40}{.013(.004)}&\cellcolor{teal!40}{.011(.001)}\\

\hline
\multirow{2}{*}{\textsc{Dutch}}&\textit{Gender}&.205(.003)&\cellcolor{teal!40}{.021(.003)}&.019(.008)&\cellcolor{teal!40}{.079(.002)}&\cellcolor{teal!40}{.008(.004)}&\cellcolor{teal!40}{.009(.005)}&\cellcolor{teal!40}{.071(.002)}&.004(.008)&\cellcolor{teal!40}{.007(.006)}\\

&\textit{Age}&\cellcolor{teal!40}{.189(.003)}&\cellcolor{teal!40}{.024(.003)}&.054(.004)&.083(.003)&.018(.002)&\cellcolor{teal!40}{.023(.002)}&.077(.002)&\cellcolor{teal!40}{.009(.003)}&\cellcolor{teal!40}{.011(.001)}\\

\hline

\multirow{3}{*}{\textsc{Credit}}&\textit{Gender}&\cellcolor{teal!40}{.179(.003)}&.033(.003)&\cellcolor{teal!40}{.021(.006)}&\cellcolor{teal!40}{.091(.002)}&\cellcolor{teal!40}{.014(.002)}&\cellcolor{teal!40}{.016(.005)}&\cellcolor{teal!40}{.069(.002)}&\cellcolor{teal!40}{.010(.001)}&\cellcolor{teal!40}{.009(.004)}\\

&\textit{Marriage}&\cellcolor{teal!40}{.182(.003)}&.028(.003)&.018(.005)&\cellcolor{teal!40}{.086(.002)}&.011(.006)&.013(.004)&.064(.002)&.008(.002)&\cellcolor{teal!40}{.010(.007)}\\

&\textit{Education}&\cellcolor{teal!40}{.186(.003)}&\cellcolor{teal!40}{.034(.003)}&\cellcolor{teal!40}{.042(.003)}&.083(.002)&.012(.004)&\cellcolor{teal!40}{.014(.001)}&\cellcolor{teal!40}{.068(.002)}&.011(.003)&\cellcolor{teal!40}{.006(.001)}\\
\hline

\multirow{2}{*}{\textsc{Crime}}&\textit{Race}&.178(.003)&\cellcolor{teal!40}{.031(.003)}&\cellcolor{teal!40}{.028(.007)}&\cellcolor{teal!40}{.089(.002)}&\cellcolor{teal!40}{.006(.005)}&.013(.005)&.063(.002)&.010(.002)&.007(.003)\\

&\textit{Gender}&\cellcolor{teal!40}{.186(.003)}&\cellcolor{teal!40}{.025(.006)}&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.086(.002)}&.011(.003)&.017(.001)&.071(.002)&.008(.003)&\cellcolor{teal!40}{.011(.001)}\\

\hline


\multirow{2}{*}{\textsc{German}}&\textit{Gender}&\cellcolor{teal!40}{.171(.003)}&.041(.002)&\cellcolor{teal!40}{.026(.008)}&\cellcolor{teal!40}{.079(.002)}&.017(.002)&\cellcolor{teal!40}{.012(.001)}&\cellcolor{teal!40}{.076(.002)}&.013(.002)&.004(.001)\\

&\textit{Age}&\cellcolor{teal!40}{.174(.003)}&\cellcolor{teal!40}{.044(.003)}&\cellcolor{teal!40}{.032(.003)}&\cellcolor{teal!40}{.084(.002)}&\cellcolor{teal!40}{.016(.002)}&\cellcolor{teal!40}{.019(.002)}&\cellcolor{teal!40}{.068(.002)}&\cellcolor{teal!40}{.009(.001)}&\cellcolor{teal!40}{.010(.002)}\\

\hline





\end{tabular}
\end{adjustbox}
\arrayrulecolor{black}
 \vspace{-0.5cm}
\end{table}

==> Table/rq4.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}[t!]
\caption{Testing the retrained DNN improved by \approach~against before retraining, without \approach, and \texttt{FairRF} over 5 retraining runs $\times$ 10 testing runs (i.e., $A-B$ where $A$ and $B$ are the metric values of testing the retrained DNN by other and \approach, respectively). All retrained samples are generated with the best generator under an approach. Positive numbers imply \approach~improves more. \setlength{\fboxsep}{1.5pt}\colorbox{teal!40}{green cells} mean the improvement is statistically significant.}

\label{tb:rq4}
\setlength{\tabcolsep}{.5mm}
\centering
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{ll|lll|lll|lll} 
\toprule

\multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{$f_s$}&\multicolumn{3}{c|}{IDI ratio (\approach~vs.)}&\multicolumn{3}{c|}{EOD (\approach~vs.)}&\multicolumn{3}{c}{SPD (\approach~vs.)}\\

\cline{3-11}

&&Before&w/o&\texttt{FairRF}&Before&w/o&\texttt{FairRF}&Before&w/o&\texttt{FairRF}\\

\midrule

\multirow{3}{*}{\textsc{Adult}}&\textit{Gender}&\cellcolor{teal!40}{.214(.002)}&\cellcolor{teal!40}{.033(.003)}&\cellcolor{teal!40}{.046(.003)}&\cellcolor{teal!40}{.084(.002)}&\cellcolor{teal!40}{.017(.002)}&\cellcolor{teal!40}{.021(.002)}&\cellcolor{teal!40}{.041(.002)}&\cellcolor{teal!40}{.012(.002)}&\cellcolor{teal!40}{.013(.002)}\\

&\textit{Race}&\cellcolor{teal!40}{.248(.003)}&\cellcolor{teal!40}{.042(.003)}&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.078(.002)}&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.029(.002)}&\cellcolor{teal!40}{.074(.002)}&\cellcolor{teal!40}{.014(.002)}&\cellcolor{teal!40}{.017(.002)}\\

&\textit{Age}&\cellcolor{teal!40}{.225(.003)}&\cellcolor{teal!40}{.036(.003)}&\cellcolor{teal!40}{.021(.006)}&\cellcolor{teal!40}{.091(.002)}&\cellcolor{teal!40}{.016(.002)}&\cellcolor{teal!40}{.013(.005)}&\cellcolor{teal!40}{.066(.002)}&\cellcolor{teal!40}{.008(.001)}&\cellcolor{teal!40}{.011(.005)}\\

\hline


\multirow{2}{*}{\textsc{Compas}}&\textit{Gender}&\cellcolor{teal!40}{.257(.003)}&\cellcolor{teal!40}{.038(.003)}&\cellcolor{teal!40}{.044(.004)}&\cellcolor{teal!40}{.081(.002)}&\cellcolor{teal!40}{.018(.002)}&\cellcolor{teal!40}{.026(.002)}&\cellcolor{teal!40}{.051(.002)}&\cellcolor{teal!40}{.014(.002)}&\cellcolor{teal!40}{.011(.002)}\\

&\textit{Race}&\cellcolor{teal!40}{.290(.003)}&\cellcolor{teal!40}{.036(.004)}&\cellcolor{teal!40}{.051(.003)}&\cellcolor{teal!40}{.092(.002)}&\cellcolor{teal!40}{.021(.003)}&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.081(.002)}&\cellcolor{teal!40}{.012(.002)}&.010(.001)\\

\hline

\multirow{2}{*}{\textsc{Law School}}&\textit{Gender}&\cellcolor{teal!40}{.235(.003)}&\cellcolor{teal!40}{.036(.003)}&\cellcolor{teal!40}{.042(.003)}&\cellcolor{teal!40}{.088(.002)}&\cellcolor{teal!40}{.019(.005)}&\cellcolor{teal!40}{.019(.001)}&\cellcolor{teal!40}{.069(.002)}&\cellcolor{teal!40}{.013(.002)}&.008(.001)\\

&\textit{Race}&\cellcolor{teal!40}{.228(.003)}&\cellcolor{teal!40}{.039(.003)}&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.077(.003)}&\cellcolor{teal!40}{.024(.003)}&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.063(.002)}&\cellcolor{teal!40}{.015(.002)}&\cellcolor{teal!40}{.011(.001)}\\

\hline


\multirow{2}{*}{\textsc{KDD}}&\textit{Gender}&\cellcolor{teal!40}{.184(.003)}&\cellcolor{teal!40}{.027(.003)}&\cellcolor{teal!40}{.037(.002)}&\cellcolor{teal!40}{.082(.002)}&\cellcolor{teal!40}{.016(.003)}&\cellcolor{teal!40}{.021(.003)}&\cellcolor{teal!40}{.061(.002)}&\cellcolor{teal!40}{.010(.002)}&\cellcolor{teal!40}{.012(.004)}\\

&\textit{Race}&\cellcolor{teal!40}{.192(.003)}&\cellcolor{teal!40}{.034(.005)}&\cellcolor{teal!40}{.052(.003)}&\cellcolor{teal!40}{.073(.002)}&\cellcolor{teal!40}{.020(.003)}&\cellcolor{teal!40}{.017(.002)}&\cellcolor{teal!40}{.064(.002)}&\cellcolor{teal!40}{.013(.004)}&\cellcolor{teal!40}{.011(.001)}\\

\hline
\multirow{2}{*}{\textsc{Dutch}}&\textit{Gender}&\cellcolor{teal!40}{.205(.003)}&\cellcolor{teal!40}{.021(.003)}&\cellcolor{teal!40}{.019(.008)}&\cellcolor{teal!40}{.079(.002)}&\cellcolor{teal!40}{.008(.004)}&\cellcolor{teal!40}{.009(.005)}&\cellcolor{teal!40}{.071(.002)}&.004(.008)&\cellcolor{teal!40}{.007(.006)}\\

&\textit{Age}&\cellcolor{teal!40}{.189(.003)}&\cellcolor{teal!40}{.024(.003)}&\cellcolor{teal!40}{.054(.004)}&\cellcolor{teal!40}{.083(.003)}&\cellcolor{teal!40}{.018(.002)}&\cellcolor{teal!40}{.023(.002)}&\cellcolor{teal!40}{.077(.002)}&\cellcolor{teal!40}{.009(.003)}&\cellcolor{teal!40}{.011(.001)}\\

\hline

\multirow{3}{*}{\textsc{Credit}}&\textit{Gender}&\cellcolor{teal!40}{.179(.003)}&\cellcolor{teal!40}{.033(.003)}&\cellcolor{teal!40}{.021(.006)}&\cellcolor{teal!40}{.091(.002)}&\cellcolor{teal!40}{.014(.002)}&\cellcolor{teal!40}{.016(.005)}&\cellcolor{teal!40}{.069(.002)}&\cellcolor{teal!40}{.010(.001)}&\cellcolor{teal!40}{.009(.004)}\\

&\textit{Marriage}&\cellcolor{teal!40}{.182(.003)}&\cellcolor{teal!40}{.028(.003)}&\cellcolor{teal!40}{.018(.005)}&\cellcolor{teal!40}{.086(.002)}&.011(.006)&\cellcolor{teal!40}{.013(.004)}&\cellcolor{teal!40}{.064(.002)}&\cellcolor{teal!40}{.008(.002)}&\cellcolor{teal!40}{.010(.007)}\\

&\textit{Education}&\cellcolor{teal!40}{.186(.003)}&\cellcolor{teal!40}{.034(.003)}&\cellcolor{teal!40}{.042(.003)}&\cellcolor{teal!40}{.083(.002)}&\cellcolor{teal!40}{.012(.004)}&\cellcolor{teal!40}{.014(.001)}&\cellcolor{teal!40}{.068(.002)}&.011(.003)&\cellcolor{teal!40}{.006(.001)}\\
\hline

\multirow{2}{*}{\textsc{Crime}}&\textit{Race}&\cellcolor{teal!40}{.178(.003)}&\cellcolor{teal!40}{.031(.003)}&\cellcolor{teal!40}{.028(.007)}&\cellcolor{teal!40}{.089(.002)}&\cellcolor{teal!40}{.006(.005)}&\cellcolor{teal!40}{.013(.005)}&\cellcolor{teal!40}{.063(.002)}&\cellcolor{teal!40}{.010(.002)}&\cellcolor{teal!40}{.007(.003)}\\

&\textit{Gender}&\cellcolor{teal!40}{.186(.003)}&\cellcolor{teal!40}{.025(.006)}&\cellcolor{teal!40}{.041(.003)}&\cellcolor{teal!40}{.086(.002)}&\cellcolor{teal!40}{.011(.003)}&\cellcolor{teal!40}{.017(.001)}&\cellcolor{teal!40}{.071(.002)}&\cellcolor{teal!40}{.008(.003)}&\cellcolor{teal!40}{.011(.001)}\\

\hline


\multirow{2}{*}{\textsc{German}}&\textit{Gender}&\cellcolor{teal!40}{.171(.003)}&\cellcolor{teal!40}{.041(.002)}&\cellcolor{teal!40}{.026(.008)}&\cellcolor{teal!40}{.079(.002)}&\cellcolor{teal!40}{.017(.002)}&\cellcolor{teal!40}{.012(.001)}&\cellcolor{teal!40}{.076(.002)}&\cellcolor{teal!40}{.013(.002)}&.004(.001)\\

&\textit{Age}&\cellcolor{teal!40}{.174(.003)}&\cellcolor{teal!40}{.044(.003)}&\cellcolor{teal!40}{.032(.003)}&\cellcolor{teal!40}{.084(.002)}&\cellcolor{teal!40}{.016(.002)}&\cellcolor{teal!40}{.019(.002)}&\cellcolor{teal!40}{.068(.002)}&\cellcolor{teal!40}{.009(.001)}&\cellcolor{teal!40}{.010(.002)}\\

\hline





\end{tabular}
\end{adjustbox}
\arrayrulecolor{black}
 %\vspace{-0.5cm}
\end{table}

==> Table/rq5.tex <==
\begin{table}[t!]
\caption{Evaluating the effect of relaxing the IDI definition and applying invalidity repair across all datasets and models. For each dataset, we report: the number of valid IDIs without relaxation, total IDIs generated under relaxation, valid and invalid counts before repair, and valid and invalid counts after repair, averaged over six generators. }
\label{tb:rq5-full1}
\setlength{\tabcolsep}{.7mm}
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{ll|rrrrrr|rrrrrr|rrrrrr}
\toprule

\multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{$f_s$}&\multicolumn{6}{c|}{\texttt{LR}}&\multicolumn{6}{c|}{\texttt{RF}}&\multicolumn{6}{c}{\texttt{DNN}}\\

\cline{3-20}
& & \multicolumn{1}{l}{w/o Relaxation} & \multicolumn{1}{l}{w/ Relaxation} 
& \multicolumn{1}{l}{Relaxation Valid} & \multicolumn{1}{l}{Relaxation Invalid} 
& \multicolumn{1}{l}{Repair Valid} & \multicolumn{1}{l|}{Repair Invalid}
& \multicolumn{1}{l}{w/o Relaxation} & \multicolumn{1}{l}{w/ Relaxation} 
& \multicolumn{1}{l}{Relaxation Valid} & \multicolumn{1}{l}{Relaxation Invalid} 
& \multicolumn{1}{l}{Repair Valid} & \multicolumn{1}{l|}{Repair Invalid}
& \multicolumn{1}{l}{w/o Relaxation} & \multicolumn{1}{l}{w/ Relaxation} 
& \multicolumn{1}{l}{Relaxation Valid} & \multicolumn{1}{l}{Relaxation Invalid} 
& \multicolumn{1}{l}{Repair Valid} & \multicolumn{1}{l|}{Repair Invalid} \\

\midrule
\multirow{3}{*}{\textsc{Adult}} & \textit{Gender}
& 1738.3 & 2898.3 & 2411.7 & 554.7 & 1798.3 & 105.4
& 1609.3 & 2795.5 & 2150.4 & 645.1 & 1716.8 & 122.7 
& 2811.7 & 4589.7 & 3906.5 & 683.2 & 3005.0 & 171.5 \\

& \textit{Race}
& 1680.0 & 2622.3 & 2222.3 & 400.0 & 1748.3 & 64.0 
& 1635.0 & 2946.8 & 2267.5 & 679.3 & 1755.0 & 169.8 
& 3216.7 & 5639.7 & 4699.7 & 940.0 & 3438.3 & 164.2 \\

& \textit{Age}
& 1566.7 & 2776.5 & 2203.5 & 573.0 & 1695.0 & 126.1 
& 1531.3 & 2677.0 & 2104.4 & 572.6 & 1641.8 & 114.5 
& 3028.3 & 5188.3 & 4198.6 & 989.7 & 3218.3 & 222.7 \\
\hline

\multirow{2}{*}{\textsc{Compas}} & \textit{Gender}
& 1618.3 & 2662.0 & 2200.0 & 462.0 & 1760.0 & 83.2 
& 1521.0 & 2526.8 & 1985.2 & 541.6 & 1583.3 & 99.0 
& 3304.2 & 5424.7 & 4608.0 & 816.7 & 3422.5 & 204.2\\

& \textit{Race}
& 1578.3 & 2918.8 & 2335.0 & 583.8 & 1716.7 & 110.9 
& 1464.0 & 2416.2 & 1932.2 & 484.0 & 1590.8 & 82.3 
& 3631.7 & 5833.4 & 4725.3 & 1108.1 & 3795.8 & 232.7 \\

\hline

\multirow{2}{*}{\textsc{Law School}} & \textit{Gender}
& 1553.3 & 2790.5 & 2163.2 & 627.3 & 1690.0 & 144.3 
& 1559.5 & 2467.4 & 1965.0 & 502.4 & 1609.0 & 88.2 
& 3035.8 & 4973.0 & 4206.2 & 766.8 & 3150.8 & 153.4 \\

& \textit{Race}
& 1561.7 & 2703.6 & 2271.9 & 431.7 & 1735.0 & 86.3 
& 1499.5 & 2397.4 & 1913.6 & 483.8 & 1543.5 & 85.7 
& 3026.7 & 5326.3 & 4359.2 & 967.1 & 3116.7 & 145.1 \\

\hline

\multirow{2}{*}{\textsc{KDD}} & \textit{Gender}
& 1551.7 & 2523.2 & 2073.6 & 352.5 & 1721.7 & 52.9 
& 1555.0 & 2530.5 & 2024.4 & 506.1 & 1588.7 & 91.1 
& 2536.7 & 4459.1 & 3816.3 & 642.8 & 2833.3 & 110.0 \\

& \textit{Race}
& 1546.7 & 2937.1 & 2407.5 & 529.6 & 1720.0 & 111.2 
& 1578.2 & 2638.2 & 2108.2 & 530.0 & 1625.5 & 95.4 
& 2545.0 & 4557.1 & 3797.6 & 759.5 & 2842.5 & 155.4 \\

\hline
\multirow{2}{*}{\textsc{Dutch}} & \textit{Gender}
& 1520.0 & 2661.2 & 2184.5 & 476.7 & 1730.0 & 91.8 
& 1653.3 & 2618.1 & 2036.9 & 581.2 & 1711.3 & 104.6 
& 2516.7 & 3954.0 & 3443.2 & 510.8 & 2846.7 & 102.2 \\

& \textit{Age}
& 1577.0 & 2821.0 & 2292.2 & 528.8 & 1790.0 & 84.6 
& 1683.8 & 2702.0 & 2077.4 & 624.6 & 1725.5 & 122.3 
& 2490.0 & 3901.0 & 3325.9 & 575.1 & 2816.7 & 103.5\\
\hline

\multirow{3}{*}{\textsc{Credit}} & \textit{Gender}
& 1577.0 & 2603.8 & 2112.4 & 491.4 & 1707.0 & 83.2 
& 1596.2 & 2560.0 & 2013.2 & 546.8 & 1662.8 & 109.4 
& 2496.7 & 3669.4 & 3112.8 & 556.6 & 2646.7 & 95.2 \\

& \textit{Marriage}
& 1517.0 & 2816.5 & 2249.3 & 567.2 & 1717.0 & 102.1 
& 1622.2 & 2624.2 & 2045.2 & 579.0 & 1655.5 & 92.6 
& 2800.0 & 4423.3 & 3664.7 & 758.6 & 2995.8 & 172.6 \\

& \textit{Education}
& 1740.0 & 3046.2 & 2437.5 & 608.7 & 1977.0 & 116.4 
& 1574.2 & 2500.6 & 1986.8 & 513.8 & 1623.8 & 103.7 
& 2641.7 & 4230.0 & 3506.7 & 723.3 & 2888.3 & 144.7 \\
\hline

\multirow{2}{*}{\textsc{Crime}} & \textit{Race}
& 1472.0 & 2485.2 & 2023.8 & 461.4 & 1638.0 & 88.7 
& 1717.0 & 2726.4 & 2134.1 & 592.3 & 1759.0 & 89.0 
& 2507.5 & 3926.1 & 3334.4 & 591.7 & 2850.0 & 118.3 \\

& \textit{Gender}
& 1712.0 & 3017.0 & 2409.8 & 607.2 & 1782.0 & 91.1 
& 1766.7 & 2811.8 & 2209.8 & 602.0 & 1816.7 & 94.3 
& 2766.7 & 4511.8 & 3694.2 & 817.6 & 3125.0 & 163.5 \\

\hline
\multirow{2}{*}{\textsc{German}} & \textit{Gender}
& 1535.2 & 2762.2 & 2191.5 & 570.7 & 1740.7 & 102.7 
& 1718.5 & 2694.6 & 2158.5 & 536.1 & 1767.0 & 80.4 
& 2623.3 & 4205.0 & 3463.5 & 741.5 & 2875.8 & 155.7 \\

& \textit{Age}
& 1536.4 & 2631.3 & 2101.0 & 530.3 & 1741.5 & 85.6 
& 1755.8 & 2765.4 & 2198.2 & 567.2 & 1809.5 & 88.1 
& 2616.7 & 4158.1 & 3462.1 & 696.0 & 2868.3 & 139.2 \\

\bottomrule
\end{tabular}
\end{adjustbox}

%\vspace{-0.4cm}
\end{table}
